Drip and Mate Operations Acting in Test Tube Systems and Tissue-like P systems

The operations drip and mate considered in (mem)brane computing resemble the operations cut and recombination well known from DNA computing. We here consider sets of vesicles with multisets of objects on their outside membrane interacting by drip and mate in two different setups: in test tube systems, the vesicles may pass from one tube to another one provided they fulfill specific constraints; in tissue-like P systems, the vesicles are immediately passed to specified cells after having undergone a drip or mate operation. In both variants, computational completeness can be obtained, yet with different constraints for the drip and mate operations.

==> eptcsdata.tex <==
\providecommand{\event}{Gabriel Ciobanu (Ed.): Membrane Computing \\
and Biologically Inspired Process Calculi 2009}
\providecommand{\volume}{11}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{123}
\providecommand{\eid}{8}

